Physics-Informed Neural Nets for Control of Dynamical Systems

Physics-informed neural networks (PINNs) impose known physical laws into the learning of deep neural networks, making sure they respect the physics of the process while decreasing the demand of labeled data. For systems represented by Ordinary Differential Equations (ODEs), the conventional PINN has a continuous time input variable and outputs the solution of the corresponding ODE. In their original form, PINNs do not allow control inputs, neither can they simulate for variable long-range intervals without serious degradation in their predictions. In this context, this work presents a new framework called Physics-Informed Neural Nets for Control (PINC), which proposes a novel PINN-based architecture that is amenable to control problems and able to simulate for longer-range time horizons that are not fixed beforehand, making it a very flexible framework when compared to traditional PINNs. Furthermore, this long-range time simulation of differential equations is faster than numerical methods since it relies only on signal propagation through the network, making it less computationally costly and, thus, a better alternative for simulation of models in Model Predictive Control. We showcase our proposal in the control of two nonlinear dynamic systems: the Van der Pol oscillator and the four-tank system.

==> comments.tex <==
\vspace{20cm}
\newpage
\section{}
\newpage
\vspace{20cm}
\newpage
\eric{---------------------------}

	 ----- Model design:
	\begin{enumerate}
		\item Train until all bias is removed. \\
		- Rescale physics informed f() function term in total loss function. \\
		- Use learning rate schedules. \\
		- Apply L-FGBS as a final training step ((when) is it necessary?) \\
		- The max time input T alllowed to the model defines a trajectory and is a design choice (T = sampling time? time to reach steady state?) \\
		- Use a sufficiently complex deep network, which easily overfits without f() for the problem at hand (e.g., 5 layers of 10, 20 neurons?) \\
		
		\eric{$N_u = 1000; N_{\mathcal{F}} = 100,000$} 
		\eric{500 épocas ADAM, 1000 iteracões L-BFGS}
		\eric{10,000 validation points }
		\\
		
		%
		- \textbf{Validation error}: use complete trajectories from casadi model only, for comparison (MSE/L2 norm over data without f() ). \\
		%
		-- \textbf{Tips}: 
		- Have a separate Python file to generate data, and save into a file. Use a function to load the data, dividing it into train/validation and test set, when the data is to be used for training/evaluating the PINN. \\
		- Most experiments below are better done in separate files, or in a way that is easily reproducible.
		%	
		\item 
		Repeat previous step, \textbf{with a fixed number of training iterations }(ADAM + L-FGBS) as in \cite{Raissi2017} (see Table 1 in \cite{Raissi2017}),
		 for different number of data $N_u$ (initial conditions and control inputs), for instance: 40, 70, 100, 500, 1.000 trajectories, and different number of collocation points $N_{\mathcal{F}}$ (2.000, 4.000, 10.000, 100.000); 
		Save validation error and total training time for each combination. Put it in table or plot. Keep T fixed (as large as reasonable);
		%
		\item Reproduce table 2 from \cite{Raissi2017} for our context, with fixed $N_u$ and $N_{\mathcal{F}}$.
		%
		\item Experiment with different $N_u$ as above (for each $N_u$, choose the best $N_{\mathcal{F}}$ from previous step), and with varying degrees of T from near to sampling time to time to reach steady state (e.g. 10 different values of T).
		For each T, save train and validation errors, as well as total training time. Use as one of the stop criteria \textit{the train/val error below some small threshold} if necessary (there should be no bias in the prediction if possible). Put it in table or plot it (surface plot: z: val error; x: T;  y: $N_u$ ). \\
		- Question here: should $N_{\mathcal{F}}$ depend on the value of T?
		%
		\item Plot model prediction with the best and worse setups found in previous step).
		\item With the best setup, vary the proportion of sampled data points (for training) between control input and time t. Plot the train/val. error in function of the proportion.
		\item Show model prediction chained by consecutive control signals with the best setup found in previous step.		
		\item 
	\end{enumerate}
	----- Data-driven discovery of unknown coefficients of ODEs:
	\begin{enumerate}
		\item Given scattered observed data (e.g., 10 trajectories with different values of unknown coefficients), treat  unknown coefficients as additional variables when minimizing MSE.
 	\end{enumerate}		
	----- Plant control:
	\begin{enumerate}
		\item  With the best model, apply NMPC in control scenarios.
	\end{enumerate}		

\vspace{1cm}
\eric{
\\ Observações:\\
- O número fixo de épocas não precisa ser grande, pois vai ter que rodar em 2 loops entrelaçados em 2 ou mais experimentos (ver tabelas 1 e 2 do artigo).
\\
-  O erro após o treinamento para construção das tabelas pode ser calculado em somente um conjunto de dados novo (assim, um deles, o de teste não é contaminado quando for selecionar o melhor par\^ametro) \\ 
- Podemos pensar, se o tempo de execução permitir, em escolher um tamanho de rede para o passo 3 acima que seja maior que o necessario, assim como fez o autor no artigo original, mostrando a capacidade de regularização do m\'etodo
\\ 
- E quanto ao passo 4 do PDF? A ideia era verificar e analisar a rela\c{c}\~ao entre $N_u$ e $T$;}


==> oilwell.tex <==
\subsubsection{Model}

\begin{figure}
    \centering
    \includegraphics{figures/well_model.eps}
    \caption{Representation of the well model employed in this work. From \cite{esmaeil}.}
    \label{fig:well_model}
\end{figure}
Oil production has many interesting applications related to control, such as slugging flow \cite{esmaeil}, or even bottom-hole pressure control for the sake of real-time optimization algorithms \cite{krishna}.
%
For this work, we employ a simplified, integral model of an oil well expressed through ordinary equations.
%
We consider a gas-lifted oil well model with two phases (gas and liquid) and two control volumes (the gas-lift annulus and the well production tubing), as depicted in Figure \ref{fig:well_model}.
%
There are two manipulated variables in the well: A production choke valve located in the wellhead, and a gas-lift valve in the gas-lift source point.
%
The model also considers load loss due to friction in its formulation, and three different boundary conditions: the reservoir pressure, the well outlet pressure, and the gas-lift source pressure.
%


The well model main state equations have the following form:
\begin{subequations}
\begin{align}
 \dot{m}_{g,a} &= \omega_{g,in} - \omega_{g,inj}\\
 \dot{m}_{g,t} &= \omega_{g,r} + \omega_{g,inj} - \omega_{g,t}\\
 \dot{m}_{l,t} &= \omega_{l,r} - \omega_{l,t}
\end{align}
\end{subequations}
These equations represent the mass flow balance between each phase, inside each control volume in the well.
%
$m_{g,a},m_{g,t},m_{l,t}$ are the well states, being the gas mass in the annulus, gas mass in the well tubing, and liquid mass in the well tubing respectively.
%
All $\omega$ correspond to mass flows, with $\omega_{g,in}$ being the gas-lift source flow, $\omega_{g,inj}$ being the mass flow coming from the gas-lift annulus to the well tubing; $\omega_{g,r}$ and $\omega{l,r}$ are the gas and liquid mass flows coming from the reservoir that the oil well is connected with; and $\omega_{l,t}$, $\omega{g,t}$ are the liquid and gas mass production flow.

Details on the full well model can be found in \cite{esmaeil}, as the full model is quite complex. 

%\subsubsection{PINC Analysis}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{PINC Control}
% N_1 = 1
% N_u = N_2, control horizon = prediction horizon
% Q = 10 * I
% R = I

% We have performed a similar approach to the first control problem with respect to finding a suitable configuration for network complexity and the proportion between data and collocation points. 
% We have observed that the minimum number of layers is 5 to get enough prediction performance for the four tanks system, since it is a more complex plant, with multiple inputs and multiple outputs (MIMO) operating at different timescales.
%
The following experiments consider a PINC net with XX layers of YY neurons each.
Besides, we continue setting
$N_t=X,000$, $N_f=Y00,000$, $K_1=X00$, and $K_2=Y0,000$.
The sampling period is $T=T_s=60s$.  
%
The control parameters are once again given by $N_1 = X$, $N_2 = X$, $N_u = N_2$, $Q = X \mathbf{I}$ and $R = \mathbf{I}$.
% validation points: 3160
% TODO: improve training plot (validation MSE)

% After training the PINC net, the prediction on test data, with new randomly generated control actions (not shown), is presented in Fig.~\ref{fig:pred_fourtanks}. The deviation in prediction at longer ranges, as seen in the first plot for $h_1$ and $h_2$, is expected, since the network works in self-loop mode, feeding its prediction of the last state back as input for the initial state (Fig.~\ref{fig:pinc_feedback}), every $T=10s$. 
% Thus, the error  is accumulated in this chaining procedure. However, MPC uses this trajectory only up to $50s$, equivalent to a prediction horizon of 5 steps, indicated by the vertical dashed line in the figure, and the next optimization procedure in MPC resets the initial state to the true value as obtained by sensors of the real process (Fig.~\ref{fig:pinc_plant}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% prediction
% \begin{figure}[tb!]
%     \centering
%     \includegraphics[width=0.49\linewidth]{figures/fourtanks_prediction_h1h2.eps}
%     \includegraphics[width=0.49\linewidth]{figures/fourtanks_prediction_h3h4.eps}
%     \caption{PINC net prediction for the four tanks system on test data, with randomly generated control input signals similar to Fig.~\ref{fig:pred_vanderpol}.
%     %The randomly generated input $u$ is given by the grey dashed line, while 
%     The predictions for the level of the tanks $h_1$ and $h_2$ correspond to the solid blue and pink lines, respectively. The target trajectories, from the RK method, are also plot in dark solid lines without dots.
%     %With a sampling time , the control action is constant during this interval. 
%     At each dot in the predicted trajectory, the PINC net receives new inputs for control action and initial state (every $T_s=T=10s$), as explained in Fig.~\ref{fig:pinc_feedback}. The vertical dashed line indicates the prediction horizon used for MPC.
%     }
%     \label{fig:pred_fourtanks}
% \end{figure}

% For this four tanks system, PINC's control employs prediction and control horizons both of 5 steps ($50s$ in simulation time). Besides, both $h_3$ and $h_4$ tank levels are constrained to the interval $[0.6, 5.5]$cm. 
% The results are shown in Fig.~\ref{fig:control_fourtanks}, where the controlled and constrained tank levels are presented in the first two topmost plots, and the control action found by MPC is shown at the bottom plot. The plots on the right-hand side show a close-up during the initial $160$s of the simulation.
% The control was successful in spite of the constrains imposed on $h_3$ and $h_4$ (which were respected) and some minor error in steady regime, which can be corrected by adding the calculation of a correction factor through filtering the error between the measurement and the network prediction, as done in \cite{Jordanou2018} for a recurrent network.
% %\cite{Plucenio2007}.
% \eb{In Fig.~\ref{fig:control_fourtanks_comparison}, we use the same simulation setup, focusing on the timesteps between 500s and 1300s, to compare with the response (in yellow color) of the control using the plant reference model as predictive model in MPC.
%   This ODE/RK-based model is the reference model that represent the plant itself, which justifies the negligible steady-state regime error observed in the figure. 
% We can notice that the PINC simulation is very close to the nominal MPC given by the ODE/RK model. We believe this comparison suffices as another NMPC would employ an approximation of the ODE/RK model as predictive model.
% }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% control
% \begin{figure}
%     \centering
%     \includegraphics[width=0.54\linewidth]{figures/fourtanks_control1.eps}
%     \includegraphics[width=0.445\linewidth]{figures/fourtanks_control_close1.eps}
%     \caption{Control of the four tanks system with PINC. 
%     %
%     The controlled variables are the tank levels $h_1$ and $h_2$ given by blue and pink lines, respectively, whereas
%     the reference trajectory for $h_1$ ($h_2$) is given by a dashed black (grey) step signal. 
%     The control inputs $\mathbf{u}$ are the manipulated voltages shown in the lower plot, found by MPC.
%     Dashed grey horizontal lines represent the lower and upper limits for both $h_3$ and $h_4$.
%     Left: simulation totalling $2400$s. Right: close-up on the first $160$s.
%     See text for more details.}
%     %
%     \label{fig:control_fourtanks}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/fourtanks_control_comparison_smallfont.eps}
%     \caption{Control of the four tanks system with PINC and the RK/ODE model for timesteps 500s to 1300s from Fig.~\ref{fig:control_fourtanks}. 
%     All the yellow lines correspond to the simulation where the ODE model itself is used as predictive model, whereas the remaining lines belong to the simulation with PINC net as predictive model.
%     }
%     \label{fig:control_fourtanks_comparison}
% \end{figure}


% The control performance in terms of RMSE and IAE is shown in Table~\ref{tab:control}. Although IAE seems to differ more between PINC and ODE/RK, RMSE errors for both methods are almost equivalent. 
% The average time spent on a desktop computer for the complete control simulation using PINC, repeated 10 times, $10.85s$, is $23.3\%$ inferior than  using the ODE of the four tanks as a model for MPC ($14.15s$), which is remarkable given the architecture of 5 hidden layers with 20 neurons each that is used for PINC.
